A Crowdsensing Approach for Deriving Surface Quality of Cycling Infrastructure

Cities worldwide are trying to increase the modal share of bicycle traffic to address traffic and carbon emission problems. Aside from safety, a key factor for this is the cycling comfort, including the surface quality of cycle paths. In this paper, we propose a novel edge-based crowdsensing method for analyzing the surface quality of bicycle paths using smartphone sensor data: Cyclists record their rides which after preprocessed on their phones before being uploaded to a private cloud backend. There, additional analysis modules aggregate data from all available rides to derive surface quality information which can then used for surface quality-aware routing and planning of infrastructure maintenance.

==> content/2_background.tex <==
%!TEX root = ../paper.tex

In this section, we give an overview of SimRa (see~\cref{sub:simra}), which provided the dataset we used in our work and of Surface Quality Analysis (see ~\cref{sub:surface_background}) in general.


\subsection{SimRa}%
\label{sub:simra}

SimRa is an open source project started in 2019 which aims to identify hotspots of near miss incidents in bicycle traffic~\cite{karakaya2020simra, temmen2022crowdsourcing}.
For this, the project follows a crowdsourcing approach in which cyclists record their daily rides using a smartphone application available for both Android and iOS.
Today, the project has managed to record more than 80,000 rides, most of them in Germany, approximately half of them in Berlin.

During the ride, SimRa records the GPS trace at 1/3Hz and the motion sensors, i.e., (linear) accelerometer, gyroscope, and rotation vector at 50Hz;
the motion sensor readings are aggregated by calculating a moving average with a window size of 30 and then keeping only every fifth value.
This was done for saving memory, battery, and mobile data usage while still being able to reconstruct the ride and detect near miss incidents.
After the ride, SimRa shows the recorded ride as a route on the map which is then annotated, cropped (for privacy reasons), and uploaded by the user.
In this paper, we only use measured data from the ride files and disregard user-annotated data on near miss incidents.

\subsection{Surface Quality Analysis}
\label{sub:surface_background}
Traffic departments frequently analyze the road surface quality to find out road segments that need to be repaired to increase the traffic safety.
There are mainly three types of methods used for, which we briefly introduce here.
\textit{Profilographs} are one of the oldest devices used to measure road surface quality.
They consist of a profiling wheel in the center and multiple support wheels held together by a rigid frame.
They measure the road quality by tracking the vertical movement of the profiling wheel.
The higher the vertical movement of that wheel, the worse the surface quality of the road.
This method of measuring surface quality is very slow, since the profilograph has to be pulled very slowly by another vehicle.
\textit{Scanner-based systems} are more sophisticated and rely either on accelerometers measuring the vibrations caused by driving on a specific surface, lasers scanning the surface in front or beneath the vehicle, cameras making photos later to be analyzed with the help of computer vision and photogrammetry, or a combination of the aforementioned methods.
This system provides the highest resolution and accuracy, however it is also the most costly and complex one.
More recently, \textit{smartphone-based systems} are gaining traction due to their cost-efficiency.
A smartphone is being attached inside the car and the vibrations caused by the road surface are recorded.
This is the least accurate system, since the measured vibrations are very indirect, due to car tires and suspension.

However, these systems are impractical for measuring bicycle road surface quality, because cars are not suited to drive on bicycle roads and these systems are too costly.
Hence, we propose a novel system using crowdsourced smartphone bicycle ride data.
